Tuning Parameter Selection for Penalized Estimation via $R^2$

The tuning parameter selection strategy for penalized estimation is crucial to identify a model that is both interpretable and predictive. However, popular strategies (e.g., minimizing average squared prediction error via cross-validation) tend to select models with more predictors than necessary. This paper proposes a simple, yet powerful cross-validation strategy based on maximizing squared correlations between the observed and predicted values, rather than minimizing squared error loss for the purposes of support recovery. The strategy can be applied to all penalized least-squares estimators and we show that, under certain conditions, the metric implicitly performs a bias adjustment. Specific attention is given to the Lasso estimator, in which our strategy is closely related to the Relaxed Lasso estimator. We demonstrate our approach on a functional variable selection problem to identify optimal placement of surface electromyogram sensors to control a robotic hand prosthesis.

==> ProofsForPaper.tex <==

\begin{proof}[Proof of Theorem~\ref{thm:AlphaGEQ1}]
Let $\hat{\boldbeta}_\lambda \neq 0$ and $g(\boldbeta) = \sum_{\ell=1}^L \lambda_\ell g_\ell(\boldbeta)$. Denote the subgradient vector of $g(\boldbeta)$ by $\nabla\V{g}^*$. Then the KKT conditions give $\frac{1}{n}\V{X}^T(\V{y} - \V{X}\hat{\boldbeta}_\lambda) = \nabla\V{g}^*$ and there exists a generalized inverse $(\V{X}^T\V{X})^{-}$ where $\hat{\boldbeta}_\lambda = (\V{X}^T\V{X})^{-}(\V{X}^T\V{y} - n \nabla\V{g}^*)$. It is easy to show $\hat{\V{y}}_\lambda^T\hat{\V{y}}_\lambda=\hat{\V{y}}_\lambda^T\V{y}- n \nabla\V{g}^{*T} \hat{\boldbeta}_\lambda$.
%Note that:
%\begin{align}
%    \hat{\V{y}}_\lambda^T\hat{\V{y}}_\lambda &= \V{y}^T \V{X}(\V{X}^T\V{X})^{-}\V{X}^T\V{y} - n\lambda \nabla\V{g}^{*T}(\V{X}^T\V{X})^{-}\V{X}^T\V{y} - n \lambda \nabla\V{g}^{*T} \hat{\boldbeta}_\lambda 
%     \ . \
%\end{align}
Therefore:
\begin{equation}
    \hat{\alpha}_\lambda =  1 + \frac{n \nabla\V{g}^{*T}\hat{\boldbeta}_\lambda}{\hat{\V{y}}_\lambda^T\hat{\V{y}}_\lambda}.
\end{equation}
Because $\hat{\V{y}}_\lambda^T\hat{\V{y}}_\lambda$, $n$, and $\lambda$ are greater than zero, we must show $\nabla\V{g}^{*T}\hat{\boldbeta}_\lambda \geq 0$. As $\nabla\V{g}^{*}$ is the subgradient of a convex function at $\hat{\boldbeta}_\lambda$, it satisfies
\begin{equation}
    %g(\boldbeta) & \geq g(\hat{\boldbeta}_\lambda) + \nabla\V{g}^{*T}(\boldbeta - \hat{\boldbeta}_\lambda)\\
    \nabla\V{g}^{*T} \hat{\boldbeta}_\lambda  \geq g(\hat{\boldbeta}_\lambda) - g(\boldbeta) + \nabla\V{g}^{*T} \boldbeta\\
\end{equation}
for all $\boldbeta$. For $\boldbeta = \V{0}$, $g(\hat{\boldbeta}_\lambda) - g(\boldbeta) + \nabla\V{g}^{*T} \boldbeta=g(\hat{\boldbeta}_\lambda) - g(\V{0}) \geq 0$. Hence, $\nabla\V{g}^{*T} \hat{\boldbeta}_\lambda \geq 0$.
% \begin{equation}
%     \nabla\V{g}^{*T} \hat{\boldbeta}_\lambda \geq g(\hat{\boldbeta}_\lambda) - g(\V{0}) \geq 0.
% \end{equation}
% Thus $\hat{\alpha}_\lambda \geq 1.$
\end{proof}


\begin{proof}[Proof of Lemma~\ref{lem:Unbiased}]
When $\boldsymbol{\xi}^*$ is recovered, we have $\hat{\boldbeta}_\lambda = \lVert \hat{\boldbeta}_\lambda \rVert_2 \boldsymbol{\xi}^*$. The response $\V{y} = \alpha^* \V{X} \boldsymbol{\xi}^* + \boldsymbol{\epsilon}$, so:
\begin{equation}
    \hat{\alpha}_\lambda \hat{\boldbeta}_\lambda = \alpha^* \boldsymbol{\xi}^* + \Big(\frac{\boldsymbol{\xi}^{*T} \V{X}^T \boldsymbol{\epsilon}}{\boldsymbol{\xi}^{*T} \V{X}^T \V{X} \boldsymbol{\xi}^*} \Big) \boldsymbol{\xi}^* \ . \
\end{equation}
Thus $E[\hat{\alpha}_\lambda \hat{\boldbeta}_\lambda] = \alpha^* \boldsymbol{\xi}^* = \boldbeta^*$.
\end{proof}

\begin{proof}[Proof of Lemma~\ref{lem:ScaledOLS}]
Fix $\lambda$ and let $\hat{\boldbeta}_\lambda = a \hat{\boldbeta}^{\mathcal{M}_\lambda}_{OLS}$ where $\hat{\boldbeta}^{\mathcal{M}_\lambda}_{OLS}$ is the OLS estimate for submodel $\mathcal{M}_\lambda$. Let $\V{X}_{\mathcal{M}_\lambda}$ be the submatrix of $\V{X}$ containing only the columns indexed by $\mathcal{M}_\lambda$. Then $\hat{\boldbeta}^{\mathcal{M}_\lambda}_{OLS} = (\V{X}_{\mathcal{M}_\lambda}^T\V{X}_{\mathcal{M}_\lambda})^{-1}\V{X}_{\mathcal{M}_\lambda}^T\V{y}$. Now: 
\begin{equation}
    \hat{\alpha}_\lambda =  \frac{a \V{y}^T \V{X}_{\mathcal{M}_\lambda}(\V{X}_{\mathcal{M}_\lambda}^T\V{X}_{\mathcal{M}_\lambda})^{-1}\V{X}_{\mathcal{M}_\lambda}^T\V{y}}{a^2 \V{y}^T \V{X}_{\mathcal{M}_\lambda}(\V{X}_{\mathcal{M}_\lambda}^T\V{X}_{\mathcal{M}_\lambda})^{-1}\V{X}_{\mathcal{M}_\lambda}^T\V{X}_{\mathcal{M}_\lambda}(\V{X}_{\mathcal{M}_\lambda}^T\V{X}_{\mathcal{M}_\lambda})^{-1}\V{X}_{\mathcal{M}_\lambda}^T\V{y}} = \frac{1}{a} \ . \
\end{equation}
Therefore:
\begin{equation}
\hat{\alpha}_\lambda \hat{\boldbeta}_\lambda = \frac{1}{a}\times a \hat{\boldbeta}_{OLS}^{ \mathcal{M}_\lambda} = \hat{\boldbeta}_{OLS}^{ \mathcal{M}_\lambda} \ . \ 
\end{equation}
\end{proof}

\begin{proof}[Proof of Theorem~\ref{thm:Consistency}]
Consider $\hat{\alpha}_{\lambda_n}:$
\begin{equation}
    \hat{\alpha}_{\lambda_n} = \frac{\frac{1}{n}\hat{\boldbeta}_{\lambda_n}^T \V{X}_n^T \V{y}}{\frac{1}{n} \hat{\boldbeta}_{\lambda_n}^T \V{X}_n^T \V{X}_n \hat{\boldbeta}_{\lambda_n}} \ . \
    \label{eq:ConsistencyEq}
\end{equation}
By Continuous Mapping Theorem, the denominator of (\ref{eq:ConsistencyEq}) converges in probability to $c^2 \boldsymbol{\xi}^{*T} \V{C} \boldsymbol{\xi}^*$. Expanding $\V{y} = \alpha^*\V{X} \boldsymbol{\xi}^* + \boldsymbol{\epsilon}$ establishes the numerator converges to $\alpha c \boldsymbol{\xi}^{*T} \V{C} \boldsymbol{\xi}^*$. Then $\hat{\alpha}_{\lambda_n} \rightarrow_p \frac{\alpha}{c}$ and  $\hat{\alpha}_{\lambda_n} \hat{\boldbeta}_{\lambda_n} \rightarrow \frac{\alpha}{c} c\boldsymbol{\xi}^* = \alpha \boldsymbol{\xi}^* = \boldbeta^*$. 
\end{proof}

% \begin{proof}[Proof of Theorem~\ref{thm:LassoConsistency}]
% \cite{LassoStrongConsistent} showed that, under the above assumptions, $\hat{\boldbeta}_{\lambda_n} \rightarrow_p \boldbeta$. By Theorem \ref{thm:Consistency}, we have the result.
% \end{proof}

% \begin{proof}[Proof of Proposition~\ref{thm:OneActive}]
% When $\hat{\boldbeta}_\lambda$ contains only one active coefficient, note that it can be written $\hat{\beta}_{\lambda,j^*}\V{v}_{j^*}$. Similarly, $\V{X}\hat{\boldbeta}_\lambda = \hat{\beta}_{\lambda,j^*}\V{X}\V{v}_{j^*} = \hat{\beta}_{\lambda,j^*} \V{X}_{j^*}$ where $\V{X}_j$ represents the $j$th column of $\V{X}$. Then:
% \begin{align}
% \alpha \hat{\boldbeta}_\lambda &= \frac{\hat{\V{y}}_\lambda^T\V{y}}{\hat{\V{y}}_\lambda^T\hat{\V{y}}_\lambda} \times \hat{\boldbeta}_\lambda = \frac{\hat{\boldbeta}_\lambda^T \V{X}^T\V{y}}{\hat{\boldbeta}_\lambda^T \V{X}^T\V{X}\hat{\boldbeta}_\lambda}\times \hat{\beta}_{\lambda,j^*}\V{v}_j\\ 
% &= \Big[\frac{\hat{\beta}_{\lambda,j^*}^2 \V{X}_j^T \V{y}}{\hat{\beta}_{\lambda,j^*}^2 \V{X}_j^T \V{X}_{j^*}}\Big]\V{v}_{j^*}= \big[(\V{X}_j^T\V{X}_{j^*})^{-1}\V{X}_{j^*}^T\V{y}\big]\V{v}_{j^*} = \hat{\beta}_{OLS,j^*} \V{v}_{j^*}.
% \end{align}
% Hence, we have the result.
% \end{proof}
% \vspace{1cm}

\begin{proof}[Proof of Theorem~\ref{thm:EModAPE}]
%APE for $K$-fold CV is calculated as:
%\begin{equation}
%      \frac{1}{K} \sum_k \frac{1}{n_k} \sum_{i} (y_{k_i} -  \V{x}_{k_i}^T\hat{\boldbeta}_\lambda)^2 . \
%\end{equation}
It is sufficient to show that $E[Mod PE] < E[PE]$ where $PE = \sum_{i} (y_{k_i} - \V{x}_{k_i}^T \hat{\boldbeta}_\lambda)^2$ and $Mod PE = \sum_{i} (y_{k_i} - \hat{\alpha}_\lambda \V{x}_{k_i}^T \hat{\boldbeta}_\lambda)^2$. We can write $\hat{\boldbeta}_\lambda=\lVert \hat{\boldbeta}_\lambda \rVert_2 \boldsymbol{\xi}^*.$ Expand $y_{k_i} = \alpha^* \V{x}_{k_i}^T \boldsymbol{\xi}^* + \epsilon_i$ to find:
\begin{equation}
    PE = \sum_i \big( \epsilon_i - \V{x}_{k_i}^T \boldsymbol{\xi}^*(\lVert \hat{\boldbeta}_\lambda \rVert_2 - \alpha^*) \big)^2 \ . \
\end{equation}
Similarly,
\begin{equation}
    Mod PE = \sum_i \Bigg( \epsilon_i - \V{x}_{k_i}^T \boldsymbol{\xi}^*\Big(\frac{\boldsymbol{\xi}^{*T}\V{X}^T \boldsymbol{\epsilon}}{\boldsymbol{\xi}^{*T}\V{X}^T \V{X} \boldsymbol{\xi}^*}\Big) \Bigg)^2 \ . \ \end{equation}
For $V(\boldsymbol{\epsilon})=\sigma^2 \V{I}$
\begin{align}
    E[PE] &= n_k \sigma^2 + \sum_i (\V{x}_{k_i}^T \boldsymbol{\xi}^*)^2 E[(\lVert \hat{\boldbeta}_\lambda \rVert_2 - \alpha)^2]\\
    E[ModPE] &= E \Bigg[ \sum_i \Bigg( \epsilon_i - \V{x}_{k_i}^T \boldsymbol{\xi}^*\Big(\frac{\boldsymbol{\xi}^{*T}\V{X}^T \boldsymbol{\epsilon}}{\boldsymbol{\xi}^{*T}\V{X}^T \V{X} \boldsymbol{\xi}^*}\Big) \Bigg)^2 \Bigg]\\
    &= n_k \sigma^2 + \sum_i \frac{(\V{x}_{k_i}^T \boldsymbol{\xi}^*)^2 E[\boldsymbol{\epsilon}^T \V{X} \boldsymbol{\xi}^* \boldsymbol{\xi}^{*T} \V{X}^T \boldsymbol{\epsilon}]}{(\boldsymbol{\xi}^{*T}\V{X}^T \V{X} \boldsymbol{\xi}^*)^2} \\
    %&= n_k \sigma^2 + \sum_i \frac{(\V{x}_{k_i}^T \boldsymbol{\xi}^*)^2 (tr(\boldsymbol{\xi}^{*T}\V{X}^T \Sigma \V{X} \boldsymbol{\xi}^*) + E[\boldsymbol{\epsilon}^T] \V{X} \boldsymbol{\xi}^* \boldsymbol{\xi}^{*T} \V{X}^T E[\boldsymbol{\epsilon}] )}{(\boldsymbol{\xi}^{*T}\V{X}^T \V{X} \boldsymbol{\xi}^*)^2} \\
    %&= n_k \sigma^2 + \sum_i \frac{(\V{x}_{k_i}^T \boldsymbol{\xi}^*)^2 \sigma^2( \boldsymbol{\xi}^{*T}\V{X}^T  \V{X} \boldsymbol{\xi}^* )}{(\boldsymbol{\xi}^{*T}\V{X}^T \V{X} \boldsymbol{\xi}^*)^2} \\
    &= n_k \sigma^2 + \frac{\sigma^2}{\boldsymbol{\xi}^{*T}\V{X}^T \V{X} \boldsymbol{\xi}^*} \sum_i (\V{x}_{k_i}^T \boldsymbol{\xi}^*)^2\ .\
\end{align}
For $\boldbeta^* = \alpha \boldsymbol{\xi}^*$, $E[PE] \geq E[ModPE]$ whenever
\begin{equation}
    E[(\lVert \hat{\boldbeta}_\lambda \rVert_2 - \alpha^*)^2] \geq \frac{\sigma^2}{\boldsymbol{\xi}^{*T}\V{X}^T \V{X} \boldsymbol{\xi}^*}
    \Leftrightarrow \frac{\alpha^{*2}}{E[(\lVert \hat{\boldbeta}_\lambda \rVert_2 - \alpha)^2]} \leq \frac{\boldbeta^{*T}\V{X}^T \V{X} \boldbeta^*}{\sigma^2}\ .\
\end{equation}
\end{proof}

\begin{proof}[Proof of Lemma~\ref{thm:AlphaBetaExpression}]
When $\V{X}$ is orthonormal,
% \begin{align}
%     \hat{\alpha}_\lambda &=  \frac{\sum_{j = 1}^p |\hat{\beta}_{OLS,j}|(|\hat{\beta}_{OLS,j}| - \lambda)_+}{\sum_{j = 1}^p (|\hat{\beta}_{OLS,j}| - \lambda)^2_+ }.
% \end{align}
% So following expression arises:
\begin{align}
    \hat{\alpha}_\lambda \hat{\beta}_{\lambda, j^*} &= \Bigg(\frac{\sum_{j = 1}^p |\hat{\beta}_{OLS,j}|(|\hat{\beta}_{OLS,j}| - \lambda)_+}{\sum_{j = 1}^p (|\hat{\beta}_{OLS,j}| - \lambda)^2_+  }\Bigg) \times \textrm{sign}(\hat{\beta}_{OLS,j^*}) \times  (|\hat{\beta}_{OLS,j^*}| - \lambda)_+\ .\
\end{align}
Letting $d_j = (|\hat{\beta}_{OLS,j}|-\lambda)_+$ and $s_{j*}=\textrm{sign}(\hat{\beta}_{OLS,j^*})$, we can rewrite this expression as
\begin{equation}
    \hat{\alpha}_\lambda \hat{\beta}_{\lambda, j^*} = w_1\hat{\beta}_{OLS,j*} + \hat{\beta}_{\lambda, j^*}\frac{\sum_{j \neq j*}(d_j+\lambda)d_j}{\sum_{j = 1}^p d_j^2}\ ,\
\end{equation}
which uses $s_{j*}|\hat{\beta}_{OLS,j*}|=\hat{\beta}_{OLS,j*}$, $w_1=d_{j*}^2/\sum_j d_j^2$, $\hat{\beta}_{\lambda, j^*}=s_{j*}d_{j*}$, and $|\hat{\beta}_{OLS,j}|=d_j+\lambda$ whenever $d_j > 0$.  Hence we have the expression
\begin{equation}
    \hat{\alpha}_\lambda \hat{\beta}_{\lambda, j^*} =w_1\hat{\beta}_{OLS,j*} + (1- w_1)\hat{\beta}_{\lambda, j^*} + w_2 \hat{\beta}_{\lambda, j^*} \ ,\
\end{equation}
where $w_2=\lambda \frac{\sum_{j \neq j*} d_j}{\sum_{j = 1}^p d_j^2}$.
\end{proof}


\begin{proof}[Proof of Theorem~\ref{thm:OrthAbsDiff}] For a given $\lambda$ we are allowing $\hat{\beta}_{OLS,j^*}$ to vary. For $|\hat{\beta}_{OLS,j^*}| \leq \lambda$, we have $\hat{\alpha}_\lambda \hat{\beta}_{\lambda,j^*}=0$ so $|\hat{\alpha}_\lambda \hat{\beta}_{\lambda,j^*} - \hat{\beta}_{OLS,j^*}| = |\hat{\beta}_{OLS,j^*}| \leq \lambda$ so the theorem is satisfied for this range of values. Next we consider $\hat{\beta}_{OLS,j^*} > \lambda$ and by Lemma~\ref{thm:AlphaBetaExpression}, and some simplification, we have
\begin{equation}
\hat{\alpha}_\lambda \hat{\beta}_{\lambda,j^*} - \hat{\beta}_{OLS,j^*} %&= (w_1 - 1) \hat{\beta}_{OLS,j^*} + (1 - w_1 + w_2) \hat{\beta}_{\lambda,j^*}\\
= \frac{\lambda (\sum_{j\neq j^*}d_j)\hat{\beta}_{OLS,j^*} - \lambda (\sum_{j\neq j^*}d_j^2 + \lambda \sum_{j\neq j^*}d_j)}{(\hat{\beta}_{OLS,j^*} - \lambda)^2 + \sum_{j\neq j^*}d_j^2}\ .\ \label{eq:Thm4ModEst}
\end{equation}
Let $u = \sum_{j\neq j^*}d_j$, $v = \sum_{j\neq j^*}d_j^2$, and $x = \hat{\beta}_{OLS,j^*}$. We can express \eqref{eq:Thm4ModEst} as $f(x) = [\lambda u x - \lambda(v + \lambda u)]/[(x - \lambda)^2 + v]$, a differentiable function for $x\geq \lambda$. Between $x=\lambda$ and $x = (u \lambda + v + \sqrt{u^2v + v^2})/u \equiv x^*$, $f(x)$ is an increasing function bounded below by $-\lambda$ and bounded above by
\begin{align}
    %\textrm{max}(f(x)) = f\Big(\frac{a \lambda + b \pm \sqrt{a^2b + b^2}}{a}\Big) = 
    \frac{\lambda}{2}\Big(\sqrt{\frac{u^2}{v } + 1 } - 1\Big)\ .\
\end{align}
For $x > x^*$, $f(x)$ is decreasing so we consider $\lim_{x \to \infty} f(x)$, which is easily shown to equal $0> -\lambda$. Therefore,
\begin{equation}
    |f(x)| \leq \lambda \times \max\left(1, \ \frac{1}{2}\Big(\sqrt{\frac{u^2}{v } + 1 } - 1\Big) \right)\ ,\
\end{equation}
and $\lim_{x \to \infty} |f(x)| = 0$. For $\hat{\beta}_{OLS,j^*} < -\lambda$, note that $\hat{\alpha}_\lambda \hat{\beta}_{\lambda,j^*} - \hat{\beta}_{OLS,j^*}=-(\hat{\alpha}_\lambda |\hat{\beta}_{\lambda,j^*}| - |\hat{\beta}_{OLS,j^*}|)$ and so analogous arguments to the case of $\hat{\beta}_{OLS,j^*}$ also apply. This completes the proof. \end{proof}

% \begin{align}
%     f(x) &= \frac{\lambda a x - \lambda(b + \lambda a)}{(x - \lambda)^2 + b}\\
%     \frac{\partial f(x)}{\partial x} &= \frac{a\lambda}{(x - \lambda)^2 + b} - \frac{2(x - \lambda)(a\lambda x - \lambda(a\lambda + b))}{((x - \lambda)^2 + b)^2} \ .\
% \end{align}
%Now we find the value of $x$ such that $\frac{\partial f(x)}{\partial x} = 0$: 






%We begin with the case where $|\hat{\alpha}_\lambda \hat{\beta}_{\lambda,j^*}| \leq |\hat{\beta}_{OLS,j^*} |$. Now, because the Lasso estimate is non-zero, $\hat{\beta}_{\lambda,j^*} = \textrm{sign}(\hat{\beta}_{OLS,j^*})(|\hat{\beta}_{OLS, j^*}| - \lambda)$ where $|\hat{\beta}_{OLS, j^*}| > \lambda$ and recall from Theorem \ref{thm:AlphaGEQ1} that $\hat{\alpha}_\lambda \geq 1$. The difference is large in this scenario when $|\hat{\alpha}_\lambda \hat{\beta}_{\lambda,j^*}|$ is small and the smallest value of $|\hat{\alpha}_\lambda \hat{\beta}_{\lambda,j^*}|$ happens when $\hat{\alpha}_\lambda = 1$ and $|\hat{\alpha}_\lambda \hat{\beta}_{\lambda,j^*} - \hat{\beta}_{OLS,j^*} | = \lambda$. 
% Then, $\hat{\alpha}_\lambda \hat{\beta}_{\lambda,j^*} = \hat{\beta}_{\lambda,j^*}$ and 
% \begin{equation}
% |\hat{\alpha}_\lambda \hat{\beta}_{\lambda,j^*} - \hat{\beta}_{OLS,j^*} | =  |\textrm{sign}(\hat{\beta}_{OLS,j^*})(|\hat{\beta}_{OLS, j^*}| - \lambda) - \hat{\beta}_{OLS,j^*}|
% =  \lambda \ . \
% \end{equation}
% Thus the largest this difference can be is $\lambda$ when the modified estimate is smaller than the OLS estimate.

%Now, we consider the case where the modified estimate is larger than the OLS estimate. 
% First, we determine what conditions lead to this occurrence: 
% \begin{equation}
%         |\hat{\beta}_{OLS,j*}| \leq |w_1 \hat{\beta}_{OLS,j^*} + (1 - w_1) \hat{\beta}_{\lambda, j^*} + w_2 \hat{\beta}_{\lambda, j^*}|.
%     \end{equation}
%By the Triangle Inequality, we have $|\hat{\beta}_{OLS,j*}| \leq |\hat{\alpha}_\lambda \hat{\beta}_{\lambda,j^*}|$ when:
%    \begin{equation}
%     |\hat{\beta}_{OLS,j*}| \leq w_1 |\hat{\beta}_{OLS,j^*}| + (1 - w_1) |\hat{\beta}_{\lambda, j^*}| + w_2 |\hat{\beta}_{\lambda, j^*}|.   
%    \end{equation}
%Note that, when $d_j \neq 0$, $|\hat{\beta}_{OLS,j}| = d_j + \lambda$. Therefore:$\frac{(1 - w_1)\lambda}{w_2} \leq d_{j^*}$.
%Hence, $|\hat{\alpha}_\lambda\hat{\beta}_{j*,\lambda}| \geq |\hat{\beta}_{OLS,j*}|$ if and only if $d_{j*} \geq \frac{\sum_{j \neq j*}d_j^2}{\sum_{j \neq j*}d_j}$. Note that when $d_{j^*} = \frac{\sum_{j\neq j^*} d_{j}^2}{\sum_{j\neq j^*} d_{j}}$, $|\hat{\alpha}_\lambda\hat{\beta}_{j*,\lambda}| = |\hat{\beta}_{OLS,j*}|$. %Now that we understand the setting in which the modified estimate surpasses the OLS estimate in magnitude, we must consider how far beyond the unbiased estimate the modified estimate might reach.
%Without loss of generality, let $\hat{\beta}_{OLS,j^*} > 0$. Now:
%\begin{equation}
%\hat{\alpha}_\lambda \hat{\beta}_{\lambda,j^*} - \hat{\beta}_{OLS,j^*} %&= (w_1 - 1) \hat{\beta}_{OLS,j^*} + (1 - w_1 + w_2) \hat{\beta}_{\lambda,j^*}\\
%= \frac{\lambda (\sum_{j\neq j^*}d_j)\hat{\beta}_{OLS,j^*} - \lambda (\sum_{j\neq j^*}d_j^2 + \lambda \sum_{j\neq j^*}d_j)}{(\hat{\beta}_{OLS,j^*} - \lambda)^2 + \sum_{j\neq j^*}d_j^2}
%\end{equation}
% Because $x > \frac{b}{a} > 0$, take the positive part of the square root. 
% By Cauchy-Swartz, we know that:
% \begin{align}
% \frac{a^2}{b} = \frac{(\sum_{j\neq j^*}d_j)^2}{\sum_{j\neq j^*}d_j^2} \leq \sum_{j\neq j^*} \frac{d_j^2}{d_j^2} = \sum_{j\neq j^*} 1 = k^*
% \end{align}
% where $k^*$ is the number of non-zero Lasso coefficients other than $j^*$. Note that when the difference between $\hat{\beta}_{OLS,j^*}$ and $\hat{\alpha}_\lambda \hat{\beta}_{\lambda,j^*}$ is greater than $\lambda$, the bias of our modified estimate is greater than the bias of the unmodified Lasso. This happens when:
% \begin{align}
%   \frac{\lambda}{2}\Big(\sqrt{\frac{a^2}{b } + 1 } - 1\Big) &> \lambda\\
%   k^* > \frac{a^2}{b} &> 8 \ .\
% \end{align}
%Therefore the bound becomes:
%\begin{align}
%   |\hat{\alpha}_\lambda \hat{\beta}_{\lambda,j^*} - \hat{\beta}_{OLS,j^*} | \leq \frac{\lambda \sqrt{( \sum_{j\neq j^*}d_j)^2(\sum_{j\neq j^*}d_j^2) + (\sum_{j\neq j^*}d_j^2)^2} - \lambda (\sum_{j\neq j^*}d_j^2)}{2(\sum_{j\neq j^*}d_j^2)} \ . \
%\end{align}
%Then when $|\hat{\alpha}_\lambda \hat{\beta}_{\lambda,j^*}| \leq |\hat{\beta}_{OLS,j^*} |$, $|\hat{\alpha}_\lambda \hat{\beta}_{\lambda,j^*} - \hat{\beta}_{OLS,j^*} | \leq \lambda$ and when $|\hat{\alpha}_\lambda \hat{\beta}_{\lambda,j^*}| > |\hat{\beta}_{OLS,j^*} |$, $|\hat{\alpha}_\lambda \hat{\beta}_{\lambda,j^*} - \hat{\beta}_{OLS,j^*} | \leq \frac{\lambda \sqrt{u^2v + v^2} - \lambda v}{2v}$ where $u = \sum_{j\neq j^*}d_j$ and $v = \sum_{j\neq j^*}d_j^2$. Therefore for any $\lambda$,
%\begin{equation}
%   |\hat{\alpha}_\lambda \hat{\beta}_{\lambda,j^*} - \hat{\beta}_{OLS,j^*} | \leq \text{max} \Big(\lambda, \frac{\lambda \sqrt{u^2v + v^2} - \lambda v}{2v} \Big) \ . \
%\end{equation} 

%Therefore we have the bound result. For the last piece, observe that $|\hat{\alpha}_\lambda\hat{\beta}_{\lambda, j^*} - \hat{\beta}_{OLS,j*}|$ is equal to:
%\begin{equation}
%        \bigl\lvert (w_1 - 1) \hat{\beta}_{OLS,j^*} + (1 - w_1) s_{j^*} (|\hat{\beta}_{OLS, j^*}|- \lambda)_+ + w_3 s_{j^*} (|\hat{\beta}_{OLS, j^*}| - \lambda)_+ \bigr\rvert \ . \
%\end{equation}
% \begin{align}
%         |\hat{\alpha}_\lambda\hat{\beta}_{\lambda, j^*} - \hat{\beta}_{OLS,j*}| &= \bigl\lvert (w_1 - 1) \hat{\beta}_{OLS,j^*} + (1 - w_1) s_{j^*} (|\hat{\beta}_{OLS, j^*}|- \lambda)_+ \\
%         & \qquad + w_3 s_{j^*} (|\hat{\beta}_{OLS, j^*}| - \lambda)_+ \bigr\rvert \ . \
% \end{align}
%It is simple to show that as $|\hat{\beta}_{OLS, j^*}|$ goes to infinity, $(w_1 - 1) \hat{\beta}_{OLS,j^*}$, $(1 - w_1) s_{j^*} (|\hat{\beta}_{OLS, j^*}| - \lambda)_+$, and $w_2 (|\hat{\beta}_{OLS,j^*}|-\lambda)_+$ all approach 0. Therefore, as $|\hat{\beta}_{OLS, j*}| \rightarrow \infty$, $|\hat{\alpha}_\lambda\hat{\beta}_{j*,\lambda} - \hat{\beta}_{OLS, j*}| \rightarrow 0$.

 
% Note that this bound may be simplified when we apply the Triangle Inequality to the first term in this expression. We find:
% \begin{align}
%   |\hat{\alpha}_\lambda \hat{\beta}_{\lambda,j^*} - \hat{\beta}_{OLS,j^*} | &\leq \frac{\lambda \Big((\sum_{j\neq j^*}d_j)\sqrt{\sum_{j\neq j^*}d_j^2} + \sum_{j\neq j^*}d_j^2 - \sum_{j\neq j^*}d_j^2  \Big)}{2(\sum_{j\neq j^*}d_j^2)}\\
%   &\leq \Big(\frac{\lambda}{2} \Big) \Bigg( \frac{\sum_{j\neq j^*}d_j}{\sqrt{\sum_{j\neq j^*}d_j^2} }\Bigg)
%   %\\
%   %& \leq \frac{\lambda}{2} \left(\frac{k\max(d_j)}{\sqrt{k\max(d_j)^2}} \right)=\frac{\lambda \sqrt{k}}{2}
% \end{align}
% We can see from this bound that as $d_j$ values become large, the bound becomes smaller for a fixed $\lambda$. That is, the larger the signals of our other covariates, the more closely the modified estimates approach the OLS estimates. This bound is especially large when $d_j$ values are close to zero.

% \begin{proof}[Proof of Corollary~\ref{thm:OrthAbsDiffGoesToInf}]
% Observe that $|\hat{\alpha}_\lambda\hat{\beta}_{\lambda, j^*} - \hat{\beta}_{OLS,j*}|$ is equal to:
% \begin{equation}
%         \bigl\lvert (w_1 - 1) \hat{\beta}_{OLS,j^*} + (1 - w_1) s_{j^*} (|\hat{\beta}_{OLS, j^*}|- \lambda)_+ + w_3 s_{j^*} (|\hat{\beta}_{OLS, j^*}| - \lambda)_+ \bigr\rvert \ . \
% \end{equation}
% % \begin{align}
% %         |\hat{\alpha}_\lambda\hat{\beta}_{\lambda, j^*} - \hat{\beta}_{OLS,j*}| &= \bigl\lvert (w_1 - 1) \hat{\beta}_{OLS,j^*} + (1 - w_1) s_{j^*} (|\hat{\beta}_{OLS, j^*}|- \lambda)_+ \\
% %         & \qquad + w_3 s_{j^*} (|\hat{\beta}_{OLS, j^*}| - \lambda)_+ \bigr\rvert \ . \
% % \end{align}
% It is simple to show that as $|\hat{\beta}_{OLS, j^*}|$ goes to infinity, $(w_1 - 1) \hat{\beta}_{OLS,j^*}$, $(1 - w_1) s_{j^*} (|\hat{\beta}_{OLS, j^*}| - \lambda)_+$, and $w_2 (|\hat{\beta}_{OLS,j^*}|-\lambda)_+$ all approach 0. Therefore, as $|\hat{\beta}_{OLS, j*}| \rightarrow \infty$, $|\hat{\alpha}_\lambda\hat{\beta}_{j*,\lambda} - \hat{\beta}_{OLS, j*}| \rightarrow 0$.
% \end{proof}


\begin{proof}[Proof of Theorem~\ref{thm:NonOrthAbsDiff}]
When the sign vector of the true model, $\V{s}$, is known there exists a closed form expression for the non-zero Lasso estimates. Let $\V{s}_1$ be the sign of the non-zero coefficient estimates and $\hat{\boldbeta}_{\lambda,1}$ be the lasso estimates for non-zero coefficients. Then $\hat{\boldbeta}_{\lambda,1} = (\hat{\boldbeta}_{OLS,1} - n\lambda (\V{X}_1^T \V{X}_1)^{-1} \V{s}_1)$ where $\V{X}_1$ is the covariate matrix including all variables $\V{s}_1$ and $\hat{\boldbeta}_{OLS,1} = (\V{X}_1^T\V{X}_1)^{-1}\V{X}_1^T\V{y}$. 
% The following is also known:
% \begin{align}
%     \hat{\alpha}_\lambda \hat{\boldbeta}_{\lambda} &= \Big( \frac{\hat{\boldbeta}_\lambda^T \V{X}_1^T \V{y} }{\hat{\boldbeta}_\lambda^T \V{X}_1^T \V{X}_1 \hat{\boldbeta}_\lambda} \Big) \hat{\boldbeta}_{\lambda}.
% \end{align}
% Now, supposing $\hat{\beta}_{\lambda,j^*} \neq 0$:
% \begin{align}
%   \hat{\V{y}}_\lambda^T \V{y}
%   &= \big( \sum_{i=1}^n x_{ij^*}^2\big)\hat{\beta}_{OLS,j^*}^2 + \big(2\sum_{i=1}^nx_{ij^*}\big(\sum_{j\neq j^*}x_{ij}\hat{\beta}_{OLS,j}\big)\big) - n\lambda s_{j^*} \big)\hat{\beta}_{OLS,j^*}\\ &\hspace{30pt} -n \lambda \sum_{j\neq j^*}|\hat{\beta}_{OLS,j}| + \sum_{i = 1}^n \big(\sum_{j\neq j^*} \hat{\beta}_{OLS,j}x_{ij} \big)^2
% %   \\
%   \end{align}
%   \begin{align}
%   \hat{\V{y}}_\lambda^T \hat{\V{y}}_\lambda &=  \big( \sum_{i=1}^n x_{ij^*}^2\big)\hat{\beta}_{OLS,j^*}^2 + \big(2\sum_{i=1}^nx_{ij^*}\big(\sum_{j\neq j^*}x_{ij}\hat{\beta}_{OLS,j}\big)\big) - 2n\lambda s_{j^*} \big)\hat{\beta}_{OLS,j^*}\\ &\hspace{30pt} -2n \lambda \sum_{j\neq j^*}|\hat{\beta}_{OLS,j}| + \sum_{i = 1}^n \big(\sum_{j\neq j^*} \hat{\beta}_{OLS,j}x_{ij} \big)^2 + n^2\lambda^2 \V{s}_1^T(\V{X}_1^T\V{X}_1)^{-1}\V{s}_1 \ . \
% \end{align} 
%When $x_{ij}$ is the $i$th element of the $j$th column of $\V{X}_1$  
Note that:
\begin{equation}
  \hat{\V{y}}_\lambda^T \V{y} - \hat{\V{y}}_\lambda^T \hat{\V{y}}_\lambda =  n\lambda s_{j^*} \hat{\beta}_{OLS,j^*} + n\lambda \sum_{j\neq j^*}|\hat{\beta}_{OLS,j}| - n^2 \lambda^2 \V{s}^T_1 (\V{X}_1^T \V{X}_1)^{-1} \V{s}_1.
\end{equation}
Hence:
\begin{equation}
    \hat{\alpha}_\lambda \hat{\beta}_{\lambda, j^*} - \hat{\beta}_{OLS, j^*}
    = \frac{(\hat{\V{y}}_\lambda^T \V{y} - \V{y}_\lambda^T \hat{\V{y}}_\lambda)\hat{\beta}_{OLS, j^*} - n\lambda\hat{\V{y}}_\lambda^T \V{y} [(\V{X}_1^T \V{X}_1)^{-1} \V{s}_1]_{j^*}}{\hat{\V{y}}_\lambda^T \hat{\V{y}}_\lambda}\ .\
\end{equation}
Using the expression for $\hat{\V{y}}_\lambda^T \V{y} - \hat{\V{y}}_\lambda^T \hat{\V{y}}_\lambda$ derived above, it can be shown that as $|\hat{\beta}_{OLS,j^*}| \rightarrow \infty$:
% \begin{equation}
%     \hat{\alpha}_\lambda \hat{\beta}_{\lambda, j^*} - \hat{\beta}_{OLS, j^*}
%     \rightarrow  n\lambda \Big( \frac{ s_{j^*}}{\big( \sum_{i=1}^n x_{ij^*}^2\big)} -[(\V{X}_1^T \V{X}_1)^{-1} \V{s}_1]_{j^*}\Big).
% \end{equation}
% If we assume that the columns of $\V{X}$ have been centered and scaled, we can say:
\begin{equation}
  \hat{\alpha}_\lambda \hat{\beta}_{\lambda, j^*} - \hat{\beta}_{OLS, j^*} \rightarrow n\lambda \Big( s_{j^*} -[(\V{X}_1^T \V{X}_1)^{-1}]_{j^*} \V{s}_1\Big) = G \ ,\
\end{equation}
where $[(\V{X}_1^T \V{X}_1)^{-1}]_{j^*}$ denotes the $j^*$-th row of $(\V{X}_1^T \V{X}_1)^{-1}$.
It is simple to show by contradiction that $\lvert G \rvert \leq \lvert \hat{\beta}_{\lambda, j^*} - \hat{\beta}_{OLS, j^*} \rvert .$ \end{proof} %Thus absolute value of the difference $\alpha$-Modified Lasso estimate and the OLS estimate approaches a constant that is always less than the absolute value of the difference between the unmodified Lasso estimate and the OLS estimate as the OLS estimate approaches infinity.





==> R2 Paper Revision/EMGFull.2.tex <==
% latex table generated in R 3.6.3 by xtable 1.8-4 package
% Tue Sep 21 09:24:50 2021
\begin{table}[ht]
\centering
\caption{Variable selection results for EMG finger movements after one stage of adaptive weighting. FP indicates the total number of false positives in the model and Size is the total number of EMG signals contained in the model.} 
\begin{tabular}{rr|ccccccc}
  \hline
 &  & FC1 & FC2 & FC3 & FR1 & FR2 & FR3 & Mean \\ 
  \hline
\multirow{3}{*}{APE} & FP & 0 & 0 & 0 & 0 & 1 & 1 & 0.33 \\ 
   & Size & 2 & 2 & 2 & 2 & 4 & 3 & 2.5 \\ 
  \multirow{3}{*}{AR2} & FP & 0 & 0 & 1 & 0 & 1 & 0 & 0.33 \\ 
   & Size & 2 & 2 & 3 & 2 & 4 & 2 & 2.5 \\ 
  \multirow{3}{*}{Mod} & FP & 0 & 0 & 0 & 0 & 1 & 1 & 0.33 \\ 
   & Size & 2 & 2 & 2 & 2 & 4 & 3 & 2.5 \\  
   \hline
\end{tabular}
\label{tab:EMGFull2}
\end{table}


==> R2 Paper Revision/EMGFull.3.tex <==
% latex table generated in R 3.6.3 by xtable 1.8-4 package
% Mon Nov 22 12:18:12 2021
\begin{table}[ht]
\centering
\caption{Variable selection results for EMG finger movements after two stages of adaptive weighting. FP indicates the total number of false positives in the model and Size is the total number of EMG signals contained in the model..} 
\begin{tabular}{rr|ccccccc}
  \hline
 &  & FC1 & FC2 & FC3 & FR1 & FR2 & FR3 & Mean \\ 
  \hline
\multirow{2}{*}{APE} & FP & 0 & 0 & 0 & 0 & 1 & 0 & 0.17 \\ 
   & Size & 2 & 2 & 2 & 2 & 4 & 2 & 2.33 \\ 
  \multirow{2}{*}{AR2} & FP & 0 & 0 & 0 & 0 & 1 & 0 & 0.17 \\ 
   & Size & 2 & 2 & 2 & 2 & 4 & 2 & 2.33 \\ 
  \multirow{2}{*}{Mod} & FP & 0 & 0 & 0 & 0 & 1 & 0 & 0.17 \\ 
   & Size & 2 & 2 & 2 & 2 & 4 & 2 & 2.33 \\ 
   \hline
\end{tabular}
\label{tab:EMGFull3}
\end{table}


==> R2 Paper Revision/EMGFull.4.tex <==
% latex table generated in R 3.6.3 by xtable 1.8-4 package
% Tue Sep 21 09:24:50 2021
\begin{table}[ht]
\centering
\caption{Variable selection results for EMG finger movements after three stages of adaptive weighting. FP indicates the total number of false positives in the model and Size is the total number of EMG signals contained in the model.} 
\begin{tabular}{rr|ccccccc}
  \hline
 &  & FC1 & FC2 & FC3 & FR1 & FR2 & FR3 & Mean \\ 
  \hline
\multirow{2}{*}{APE} & FP & 0 & 0 & 0 & 0 & 0 & 0 & 0 \\ 
   & Size & 2 & 2 & 2 & 2 & 3 & 2 & 2.17 \\ 
  \multirow{2}{*}{AR2}  & FP & 0 & 0 & 0 & 0 &  1 & 0 & 0.17 \\ 
   & Size & 2 & 2 & 2 & 2 &  4 & 2 & 2.33 \\ 
  \multirow{2}{*}{Mod}  & FP & 0 & 0 & 0 & 0 & 0 & 0 & 0 \\ 
   & Size & 2 & 2 & 2 & 2 & 3 & 2 & 2.17 \\ 
   \hline
\end{tabular}
\label{tab:EMGFull4}
\end{table}

==> R2 Paper Revision/EMGFull.5.tex <==
% latex table generated in R 3.6.3 by xtable 1.8-4 package
% Fri Oct  1 09:50:14 2021
\begin{table}[ht]
\centering
\caption{Variable selection results for EMG finger movements after the four stages of adaptive weighting recommended by \cite{SAFE}. FP indicates the total number of false positives in the model and Size is the total number of EMG signals contained in the model.}
\begin{tabular}{rr|ccccccc}
  \hline
 &  & FC1 & FC2 & FC3 & FR1 & FR2 & FR3 & Mean \\ 
  \hline
\multirow{2}{*}{APE} & FP & 0 & 0 & 0 & 0 & 0 & 0 & 0 \\ 
   & Size & 2 & 2 & 2 & 2 & 3 & 2 & 2.17 \\ 
  \multirow{2}{*}{AR2}  & FP & 0 & 0 & 0 & 0 & 1 & 0 & 0.17 \\ 
   & Size & 2 & 2 & 2 & 2 &  4 & 2 & 2.33 \\ 
  \multirow{2}{*}{Mod}  & FP & 0 & 0 & 0 & 0 & 0 & 0 & 0 \\ 
   & Size & 2 & 2 & 2 & 2 & 3 & 2 & 2.17 \\ 
   \hline
\end{tabular}
\label{tab:EMGFull5}
\end{table}


==> R2 Paper Revision/ProofsForPaper.tex <==

\begin{proof}[Proof of Theorem~\ref{thm:AlphaGEQ1}]
Let $\hat{\boldbeta}_\lambda \neq 0$ and $g(\boldbeta) = \sum_{\ell=1}^L \lambda_\ell g_\ell(\boldbeta)$. Denote the subgradient vector of $g(\boldbeta)$ by $\nabla\V{g}^*$. Then the KKT conditions give $\frac{1}{n}\V{X}^T(\V{y} - \V{X}\hat{\boldbeta}_\lambda) = \nabla\V{g}^*$ and there exists a generalized inverse $(\V{X}^T\V{X})^{-}$ where $\hat{\boldbeta}_\lambda = (\V{X}^T\V{X})^{-}(\V{X}^T\V{y} - n \nabla\V{g}^*)$. It is easy to show $\hat{\V{y}}_\lambda^T\hat{\V{y}}_\lambda=\hat{\V{y}}_\lambda^T\V{y}- n \nabla\V{g}^{*T} \hat{\boldbeta}_\lambda$.
%Note that:
%\begin{align}
%    \hat{\V{y}}_\lambda^T\hat{\V{y}}_\lambda &= \V{y}^T \V{X}(\V{X}^T\V{X})^{-}\V{X}^T\V{y} - n\lambda \nabla\V{g}^{*T}(\V{X}^T\V{X})^{-}\V{X}^T\V{y} - n \lambda \nabla\V{g}^{*T} \hat{\boldbeta}_\lambda 
%     \ . \
%\end{align}
Therefore:
\begin{equation}
    \hat{\alpha}_\lambda =  1 + \frac{n \nabla\V{g}^{*T}\hat{\boldbeta}_\lambda}{\hat{\V{y}}_\lambda^T\hat{\V{y}}_\lambda}.
\end{equation}
Because $\hat{\V{y}}_\lambda^T\hat{\V{y}}_\lambda$, $n$, and $\lambda$ are greater than zero, we must show $\nabla\V{g}^{*T}\hat{\boldbeta}_\lambda \geq 0$. As $\nabla\V{g}^{*}$ is the subgradient of a convex function at $\hat{\boldbeta}_\lambda$, it satisfies
\begin{equation}
    %g(\boldbeta) & \geq g(\hat{\boldbeta}_\lambda) + \nabla\V{g}^{*T}(\boldbeta - \hat{\boldbeta}_\lambda)\\
    \nabla\V{g}^{*T} \hat{\boldbeta}_\lambda  \geq g(\hat{\boldbeta}_\lambda) - g(\boldbeta) + \nabla\V{g}^{*T} \boldbeta\\
\end{equation}
for all $\boldbeta$. For $\boldbeta = \V{0}$, $g(\hat{\boldbeta}_\lambda) - g(\boldbeta) + \nabla\V{g}^{*T} \boldbeta=g(\hat{\boldbeta}_\lambda) - g(\V{0}) \geq 0$. Hence, $\nabla\V{g}^{*T} \hat{\boldbeta}_\lambda \geq 0$.
% \begin{equation}
%     \nabla\V{g}^{*T} \hat{\boldbeta}_\lambda \geq g(\hat{\boldbeta}_\lambda) - g(\V{0}) \geq 0.
% \end{equation}
% Thus $\hat{\alpha}_\lambda \geq 1.$
\end{proof}


\begin{proof}[Proof of Lemma~\ref{lem:Unbiased}]
When $\boldsymbol{\xi}^*$ is recovered, we have $\hat{\boldbeta}_\lambda = \lVert \hat{\boldbeta}_\lambda \rVert_2 \boldsymbol{\xi}^*$. The response $\V{y} = \alpha^* \V{X} \boldsymbol{\xi}^* + \boldsymbol{\epsilon}$, so:
\begin{equation}
    \hat{\alpha}_\lambda \hat{\boldbeta}_\lambda = \alpha^* \boldsymbol{\xi}^* + \Big(\frac{\boldsymbol{\xi}^{*T} \V{X}^T \boldsymbol{\epsilon}}{\boldsymbol{\xi}^{*T} \V{X}^T \V{X} \boldsymbol{\xi}^*} \Big) \boldsymbol{\xi}^* \ . \
\end{equation}
Thus $E[\hat{\alpha}_\lambda \hat{\boldbeta}_\lambda] = \alpha^* \boldsymbol{\xi}^* = \boldbeta^*$.
\end{proof}

\begin{proof}[Proof of Lemma~\ref{lem:ScaledOLS}]
Fix $\lambda$ and let $\hat{\boldbeta}_\lambda = a \hat{\boldbeta}^{\mathcal{M}_\lambda}_{OLS}$ where $\hat{\boldbeta}^{\mathcal{M}_\lambda}_{OLS}$ is the OLS estimate for submodel $\mathcal{M}_\lambda$. Let $\V{X}_{\mathcal{M}_\lambda}$ be the submatrix of $\V{X}$ containing only the columns indexed by $\mathcal{M}_\lambda$. Then $\hat{\boldbeta}^{\mathcal{M}_\lambda}_{OLS} = (\V{X}_{\mathcal{M}_\lambda}^T\V{X}_{\mathcal{M}_\lambda})^{-1}\V{X}_{\mathcal{M}_\lambda}^T\V{y}$. Now: 
\begin{equation}
    \hat{\alpha}_\lambda =  \frac{a \V{y}^T \V{X}_{\mathcal{M}_\lambda}(\V{X}_{\mathcal{M}_\lambda}^T\V{X}_{\mathcal{M}_\lambda})^{-1}\V{X}_{\mathcal{M}_\lambda}^T\V{y}}{a^2 \V{y}^T \V{X}_{\mathcal{M}_\lambda}(\V{X}_{\mathcal{M}_\lambda}^T\V{X}_{\mathcal{M}_\lambda})^{-1}\V{X}_{\mathcal{M}_\lambda}^T\V{X}_{\mathcal{M}_\lambda}(\V{X}_{\mathcal{M}_\lambda}^T\V{X}_{\mathcal{M}_\lambda})^{-1}\V{X}_{\mathcal{M}_\lambda}^T\V{y}} = \frac{1}{a} \ . \
\end{equation}
Therefore:
\begin{equation}
\hat{\alpha}_\lambda \hat{\boldbeta}_\lambda = \frac{1}{a}\times a \hat{\boldbeta}_{OLS}^{ \mathcal{M}_\lambda} = \hat{\boldbeta}_{OLS}^{ \mathcal{M}_\lambda} \ . \ 
\end{equation}
\end{proof}

\begin{proof}[Proof of Theorem~\ref{thm:Consistency}]
Consider $\hat{\alpha}_{\lambda_n}:$
\begin{equation}
    \hat{\alpha}_{\lambda_n} = \frac{\frac{1}{n}\hat{\boldbeta}_{\lambda_n}^T \V{X}_n^T \V{y}}{\frac{1}{n} \hat{\boldbeta}_{\lambda_n}^T \V{X}_n^T \V{X}_n \hat{\boldbeta}_{\lambda_n}} \ . \
    \label{eq:ConsistencyEq}
\end{equation}
By Continuous Mapping Theorem, the denominator of (\ref{eq:ConsistencyEq}) converges in probability to $c^2 \boldsymbol{\xi}^{*T} \V{C} \boldsymbol{\xi}^*$. Expanding $\V{y} = \alpha^*\V{X} \boldsymbol{\xi}^* + \boldsymbol{\epsilon}$ establishes the numerator converges to $\alpha c \boldsymbol{\xi}^{*T} \V{C} \boldsymbol{\xi}^*$. Then $\hat{\alpha}_{\lambda_n} \rightarrow_p \frac{\alpha}{c}$ and  $\hat{\alpha}_{\lambda_n} \hat{\boldbeta}_{\lambda_n} \rightarrow \frac{\alpha}{c} c\boldsymbol{\xi}^* = \alpha \boldsymbol{\xi}^* = \boldbeta^*$. 
\end{proof}

% \begin{proof}[Proof of Theorem~\ref{thm:LassoConsistency}]
% \cite{LassoStrongConsistent} showed that, under the above assumptions, $\hat{\boldbeta}_{\lambda_n} \rightarrow_p \boldbeta$. By Theorem \ref{thm:Consistency}, we have the result.
% \end{proof}

% \begin{proof}[Proof of Proposition~\ref{thm:OneActive}]
% When $\hat{\boldbeta}_\lambda$ contains only one active coefficient, note that it can be written $\hat{\beta}_{\lambda,j^*}\V{v}_{j^*}$. Similarly, $\V{X}\hat{\boldbeta}_\lambda = \hat{\beta}_{\lambda,j^*}\V{X}\V{v}_{j^*} = \hat{\beta}_{\lambda,j^*} \V{X}_{j^*}$ where $\V{X}_j$ represents the $j$th column of $\V{X}$. Then:
% \begin{align}
% \alpha \hat{\boldbeta}_\lambda &= \frac{\hat{\V{y}}_\lambda^T\V{y}}{\hat{\V{y}}_\lambda^T\hat{\V{y}}_\lambda} \times \hat{\boldbeta}_\lambda = \frac{\hat{\boldbeta}_\lambda^T \V{X}^T\V{y}}{\hat{\boldbeta}_\lambda^T \V{X}^T\V{X}\hat{\boldbeta}_\lambda}\times \hat{\beta}_{\lambda,j^*}\V{v}_j\\ 
% &= \Big[\frac{\hat{\beta}_{\lambda,j^*}^2 \V{X}_j^T \V{y}}{\hat{\beta}_{\lambda,j^*}^2 \V{X}_j^T \V{X}_{j^*}}\Big]\V{v}_{j^*}= \big[(\V{X}_j^T\V{X}_{j^*})^{-1}\V{X}_{j^*}^T\V{y}\big]\V{v}_{j^*} = \hat{\beta}_{OLS,j^*} \V{v}_{j^*}.
% \end{align}
% Hence, we have the result.
% \end{proof}
% \vspace{1cm}

\begin{proof}[Proof of Theorem~\ref{thm:EModAPE}]
%APE for $K$-fold CV is calculated as:
%\begin{equation}
%      \frac{1}{K} \sum_k \frac{1}{n_k} \sum_{i} (y_{k_i} -  \V{x}_{k_i}^T\hat{\boldbeta}_\lambda)^2 . \
%\end{equation}
It is sufficient to show that $E[Mod PE] < E[PE]$ where $PE = \sum_{i} (y_{k_i} - \V{x}_{k_i}^T \hat{\boldbeta}_\lambda)^2$ and $Mod PE = \sum_{i} (y_{k_i} - \hat{\alpha}_\lambda \V{x}_{k_i}^T \hat{\boldbeta}_\lambda)^2$. We can write $\hat{\boldbeta}_\lambda=\lVert \hat{\boldbeta}_\lambda \rVert_2 \boldsymbol{\xi}^*.$ Expand $y_{k_i} = \alpha^* \V{x}_{k_i}^T \boldsymbol{\xi}^* + \epsilon_i$ to find:
\begin{equation}
    PE = \sum_i \big( \epsilon_i - \V{x}_{k_i}^T \boldsymbol{\xi}^*(\lVert \hat{\boldbeta}_\lambda \rVert_2 - \alpha^*) \big)^2 \ . \
\end{equation}
Similarly,
\begin{equation}
    Mod PE = \sum_i \Bigg( \epsilon_i - \V{x}_{k_i}^T \boldsymbol{\xi}^*\Big(\frac{\boldsymbol{\xi}^{*T}\V{X}^T \boldsymbol{\epsilon}}{\boldsymbol{\xi}^{*T}\V{X}^T \V{X} \boldsymbol{\xi}^*}\Big) \Bigg)^2 \ . \ \end{equation}
For $V(\boldsymbol{\epsilon})=\sigma^2 \V{I}$
\begin{align}
    E[PE] &= n_k \sigma^2 + \sum_i (\V{x}_{k_i}^T \boldsymbol{\xi}^*)^2 E[(\lVert \hat{\boldbeta}_\lambda \rVert_2 - \alpha)^2]\\
    E[ModPE] &= E \Bigg[ \sum_i \Bigg( \epsilon_i - \V{x}_{k_i}^T \boldsymbol{\xi}^*\Big(\frac{\boldsymbol{\xi}^{*T}\V{X}^T \boldsymbol{\epsilon}}{\boldsymbol{\xi}^{*T}\V{X}^T \V{X} \boldsymbol{\xi}^*}\Big) \Bigg)^2 \Bigg]\\
    &= n_k \sigma^2 + \sum_i \frac{(\V{x}_{k_i}^T \boldsymbol{\xi}^*)^2 E[\boldsymbol{\epsilon}^T \V{X} \boldsymbol{\xi}^* \boldsymbol{\xi}^{*T} \V{X}^T \boldsymbol{\epsilon}]}{(\boldsymbol{\xi}^{*T}\V{X}^T \V{X} \boldsymbol{\xi}^*)^2} \\
    %&= n_k \sigma^2 + \sum_i \frac{(\V{x}_{k_i}^T \boldsymbol{\xi}^*)^2 (tr(\boldsymbol{\xi}^{*T}\V{X}^T \Sigma \V{X} \boldsymbol{\xi}^*) + E[\boldsymbol{\epsilon}^T] \V{X} \boldsymbol{\xi}^* \boldsymbol{\xi}^{*T} \V{X}^T E[\boldsymbol{\epsilon}] )}{(\boldsymbol{\xi}^{*T}\V{X}^T \V{X} \boldsymbol{\xi}^*)^2} \\
    %&= n_k \sigma^2 + \sum_i \frac{(\V{x}_{k_i}^T \boldsymbol{\xi}^*)^2 \sigma^2( \boldsymbol{\xi}^{*T}\V{X}^T  \V{X} \boldsymbol{\xi}^* )}{(\boldsymbol{\xi}^{*T}\V{X}^T \V{X} \boldsymbol{\xi}^*)^2} \\
    &= n_k \sigma^2 + \frac{\sigma^2}{\boldsymbol{\xi}^{*T}\V{X}^T \V{X} \boldsymbol{\xi}^*} \sum_i (\V{x}_{k_i}^T \boldsymbol{\xi}^*)^2\ .\
\end{align}
For $\boldbeta^* = \alpha \boldsymbol{\xi}^*$, $E[PE] \geq E[ModPE]$ whenever
\begin{equation}
    E[(\lVert \hat{\boldbeta}_\lambda \rVert_2 - \alpha^*)^2] \geq \frac{\sigma^2}{\boldsymbol{\xi}^{*T}\V{X}^T \V{X} \boldsymbol{\xi}^*}
    \Leftrightarrow \frac{\alpha^{*2}}{E[(\lVert \hat{\boldbeta}_\lambda \rVert_2 - \alpha)^2]} \leq \frac{\boldbeta^{*T}\V{X}^T \V{X} \boldbeta^*}{\sigma^2}\ .\
\end{equation}
\end{proof}

\begin{proof}[Proof of Lemma~\ref{thm:AlphaBetaExpression}]
When $\V{X}$ is orthonormal,
% \begin{align}
%     \hat{\alpha}_\lambda &=  \frac{\sum_{j = 1}^p |\hat{\beta}_{OLS,j}|(|\hat{\beta}_{OLS,j}| - \lambda)_+}{\sum_{j = 1}^p (|\hat{\beta}_{OLS,j}| - \lambda)^2_+ }.
% \end{align}
% So following expression arises:
\begin{align}
    \hat{\alpha}_\lambda \hat{\beta}_{\lambda, j^*} &= \Bigg(\frac{\sum_{j = 1}^p |\hat{\beta}_{OLS,j}|(|\hat{\beta}_{OLS,j}| - \lambda)_+}{\sum_{j = 1}^p (|\hat{\beta}_{OLS,j}| - \lambda)^2_+  }\Bigg) \times \textrm{sign}(\hat{\beta}_{OLS,j^*}) \times  (|\hat{\beta}_{OLS,j^*}| - \lambda)_+\ .\
\end{align}
Letting $d_j = (|\hat{\beta}_{OLS,j}|-\lambda)_+$ and $s_{j*}=\textrm{sign}(\hat{\beta}_{OLS,j^*})$, we can rewrite this expression as
\begin{equation}
    \hat{\alpha}_\lambda \hat{\beta}_{\lambda, j^*} = w_1\hat{\beta}_{OLS,j*} + \hat{\beta}_{\lambda, j^*}\frac{\sum_{j \neq j*}(d_j+\lambda)d_j}{\sum_{j = 1}^p d_j^2}\ ,\
\end{equation}
which uses $s_{j*}|\hat{\beta}_{OLS,j*}|=\hat{\beta}_{OLS,j*}$, $w_1=d_{j*}^2/\sum_j d_j^2$, $\hat{\beta}_{\lambda, j^*}=s_{j*}d_{j*}$, and $|\hat{\beta}_{OLS,j}|=d_j+\lambda$ whenever $d_j > 0$.  Hence we have the expression
\begin{equation}
    \hat{\alpha}_\lambda \hat{\beta}_{\lambda, j^*} =w_1\hat{\beta}_{OLS,j*} + (1- w_1)\hat{\beta}_{\lambda, j^*} + w_2 \hat{\beta}_{\lambda, j^*} \ ,\
\end{equation}
where $w_2=\lambda \frac{\sum_{j \neq j*} d_j}{\sum_{j = 1}^p d_j^2}$.
\end{proof}


\begin{proof}[Proof of Theorem~\ref{thm:OrthAbsDiff}] For a given $\lambda$ we are allowing $\hat{\beta}_{OLS,j^*}$ to vary. For $|\hat{\beta}_{OLS,j^*}| \leq \lambda$, we have $\hat{\alpha}_\lambda \hat{\beta}_{\lambda,j^*}=0$ so $|\hat{\alpha}_\lambda \hat{\beta}_{\lambda,j^*} - \hat{\beta}_{OLS,j^*}| = |\hat{\beta}_{OLS,j^*}| \leq \lambda$ so the theorem is satisfied for this range of values. Next we consider $\hat{\beta}_{OLS,j^*} > \lambda$ and by Lemma~\ref{thm:AlphaBetaExpression}, and some simplification, we have
\begin{equation}
\hat{\alpha}_\lambda \hat{\beta}_{\lambda,j^*} - \hat{\beta}_{OLS,j^*} %&= (w_1 - 1) \hat{\beta}_{OLS,j^*} + (1 - w_1 + w_2) \hat{\beta}_{\lambda,j^*}\\
= \frac{\lambda (\sum_{j\neq j^*}d_j)\hat{\beta}_{OLS,j^*} - \lambda (\sum_{j\neq j^*}d_j^2 + \lambda \sum_{j\neq j^*}d_j)}{(\hat{\beta}_{OLS,j^*} - \lambda)^2 + \sum_{j\neq j^*}d_j^2}\ .\ \label{eq:Thm4ModEst}
\end{equation}
Let $u = \sum_{j\neq j^*}d_j$, $v = \sum_{j\neq j^*}d_j^2$, and $x = \hat{\beta}_{OLS,j^*}$. We can express \eqref{eq:Thm4ModEst} as $f(x) = [\lambda u x - \lambda(v + \lambda u)]/[(x - \lambda)^2 + v]$, a differentiable function for $x\geq \lambda$. Between $x=\lambda$ and $x = (u \lambda + v + \sqrt{u^2v + v^2})/u \equiv x^*$, $f(x)$ is an increasing function bounded below by $-\lambda$ and bounded above by
\begin{align}
    %\textrm{max}(f(x)) = f\Big(\frac{a \lambda + b \pm \sqrt{a^2b + b^2}}{a}\Big) = 
    \frac{\lambda}{2}\Big(\sqrt{\frac{u^2}{v } + 1 } - 1\Big)\ .\
\end{align}
For $x > x^*$, $f(x)$ is decreasing so we consider $\lim_{x \to \infty} f(x)$, which is easily shown to equal $0> -\lambda$. Therefore,
\begin{equation}
    |f(x)| \leq \lambda \times \max\left(1, \ \frac{1}{2}\Big(\sqrt{\frac{u^2}{v } + 1 } - 1\Big) \right)\ ,\
\end{equation}
and $\lim_{x \to \infty} |f(x)| = 0$. For $\hat{\beta}_{OLS,j^*} < -\lambda$, note that $\hat{\alpha}_\lambda \hat{\beta}_{\lambda,j^*} - \hat{\beta}_{OLS,j^*}=-(\hat{\alpha}_\lambda |\hat{\beta}_{\lambda,j^*}| - |\hat{\beta}_{OLS,j^*}|)$ and so analogous arguments to the case of $\hat{\beta}_{OLS,j^*}$ also apply. This completes the proof. \end{proof}

% \begin{align}
%     f(x) &= \frac{\lambda a x - \lambda(b + \lambda a)}{(x - \lambda)^2 + b}\\
%     \frac{\partial f(x)}{\partial x} &= \frac{a\lambda}{(x - \lambda)^2 + b} - \frac{2(x - \lambda)(a\lambda x - \lambda(a\lambda + b))}{((x - \lambda)^2 + b)^2} \ .\
% \end{align}
%Now we find the value of $x$ such that $\frac{\partial f(x)}{\partial x} = 0$: 






%We begin with the case where $|\hat{\alpha}_\lambda \hat{\beta}_{\lambda,j^*}| \leq |\hat{\beta}_{OLS,j^*} |$. Now, because the Lasso estimate is non-zero, $\hat{\beta}_{\lambda,j^*} = \textrm{sign}(\hat{\beta}_{OLS,j^*})(|\hat{\beta}_{OLS, j^*}| - \lambda)$ where $|\hat{\beta}_{OLS, j^*}| > \lambda$ and recall from Theorem \ref{thm:AlphaGEQ1} that $\hat{\alpha}_\lambda \geq 1$. The difference is large in this scenario when $|\hat{\alpha}_\lambda \hat{\beta}_{\lambda,j^*}|$ is small and the smallest value of $|\hat{\alpha}_\lambda \hat{\beta}_{\lambda,j^*}|$ happens when $\hat{\alpha}_\lambda = 1$ and $|\hat{\alpha}_\lambda \hat{\beta}_{\lambda,j^*} - \hat{\beta}_{OLS,j^*} | = \lambda$. 
% Then, $\hat{\alpha}_\lambda \hat{\beta}_{\lambda,j^*} = \hat{\beta}_{\lambda,j^*}$ and 
% \begin{equation}
% |\hat{\alpha}_\lambda \hat{\beta}_{\lambda,j^*} - \hat{\beta}_{OLS,j^*} | =  |\textrm{sign}(\hat{\beta}_{OLS,j^*})(|\hat{\beta}_{OLS, j^*}| - \lambda) - \hat{\beta}_{OLS,j^*}|
% =  \lambda \ . \
% \end{equation}
% Thus the largest this difference can be is $\lambda$ when the modified estimate is smaller than the OLS estimate.

%Now, we consider the case where the modified estimate is larger than the OLS estimate. 
% First, we determine what conditions lead to this occurrence: 
% \begin{equation}
%         |\hat{\beta}_{OLS,j*}| \leq |w_1 \hat{\beta}_{OLS,j^*} + (1 - w_1) \hat{\beta}_{\lambda, j^*} + w_2 \hat{\beta}_{\lambda, j^*}|.
%     \end{equation}
%By the Triangle Inequality, we have $|\hat{\beta}_{OLS,j*}| \leq |\hat{\alpha}_\lambda \hat{\beta}_{\lambda,j^*}|$ when:
%    \begin{equation}
%     |\hat{\beta}_{OLS,j*}| \leq w_1 |\hat{\beta}_{OLS,j^*}| + (1 - w_1) |\hat{\beta}_{\lambda, j^*}| + w_2 |\hat{\beta}_{\lambda, j^*}|.   
%    \end{equation}
%Note that, when $d_j \neq 0$, $|\hat{\beta}_{OLS,j}| = d_j + \lambda$. Therefore:$\frac{(1 - w_1)\lambda}{w_2} \leq d_{j^*}$.
%Hence, $|\hat{\alpha}_\lambda\hat{\beta}_{j*,\lambda}| \geq |\hat{\beta}_{OLS,j*}|$ if and only if $d_{j*} \geq \frac{\sum_{j \neq j*}d_j^2}{\sum_{j \neq j*}d_j}$. Note that when $d_{j^*} = \frac{\sum_{j\neq j^*} d_{j}^2}{\sum_{j\neq j^*} d_{j}}$, $|\hat{\alpha}_\lambda\hat{\beta}_{j*,\lambda}| = |\hat{\beta}_{OLS,j*}|$. %Now that we understand the setting in which the modified estimate surpasses the OLS estimate in magnitude, we must consider how far beyond the unbiased estimate the modified estimate might reach.
%Without loss of generality, let $\hat{\beta}_{OLS,j^*} > 0$. Now:
%\begin{equation}
%\hat{\alpha}_\lambda \hat{\beta}_{\lambda,j^*} - \hat{\beta}_{OLS,j^*} %&= (w_1 - 1) \hat{\beta}_{OLS,j^*} + (1 - w_1 + w_2) \hat{\beta}_{\lambda,j^*}\\
%= \frac{\lambda (\sum_{j\neq j^*}d_j)\hat{\beta}_{OLS,j^*} - \lambda (\sum_{j\neq j^*}d_j^2 + \lambda \sum_{j\neq j^*}d_j)}{(\hat{\beta}_{OLS,j^*} - \lambda)^2 + \sum_{j\neq j^*}d_j^2}
%\end{equation}
% Because $x > \frac{b}{a} > 0$, take the positive part of the square root. 
% By Cauchy-Swartz, we know that:
% \begin{align}
% \frac{a^2}{b} = \frac{(\sum_{j\neq j^*}d_j)^2}{\sum_{j\neq j^*}d_j^2} \leq \sum_{j\neq j^*} \frac{d_j^2}{d_j^2} = \sum_{j\neq j^*} 1 = k^*
% \end{align}
% where $k^*$ is the number of non-zero Lasso coefficients other than $j^*$. Note that when the difference between $\hat{\beta}_{OLS,j^*}$ and $\hat{\alpha}_\lambda \hat{\beta}_{\lambda,j^*}$ is greater than $\lambda$, the bias of our modified estimate is greater than the bias of the unmodified Lasso. This happens when:
% \begin{align}
%   \frac{\lambda}{2}\Big(\sqrt{\frac{a^2}{b } + 1 } - 1\Big) &> \lambda\\
%   k^* > \frac{a^2}{b} &> 8 \ .\
% \end{align}
%Therefore the bound becomes:
%\begin{align}
%   |\hat{\alpha}_\lambda \hat{\beta}_{\lambda,j^*} - \hat{\beta}_{OLS,j^*} | \leq \frac{\lambda \sqrt{( \sum_{j\neq j^*}d_j)^2(\sum_{j\neq j^*}d_j^2) + (\sum_{j\neq j^*}d_j^2)^2} - \lambda (\sum_{j\neq j^*}d_j^2)}{2(\sum_{j\neq j^*}d_j^2)} \ . \
%\end{align}
%Then when $|\hat{\alpha}_\lambda \hat{\beta}_{\lambda,j^*}| \leq |\hat{\beta}_{OLS,j^*} |$, $|\hat{\alpha}_\lambda \hat{\beta}_{\lambda,j^*} - \hat{\beta}_{OLS,j^*} | \leq \lambda$ and when $|\hat{\alpha}_\lambda \hat{\beta}_{\lambda,j^*}| > |\hat{\beta}_{OLS,j^*} |$, $|\hat{\alpha}_\lambda \hat{\beta}_{\lambda,j^*} - \hat{\beta}_{OLS,j^*} | \leq \frac{\lambda \sqrt{u^2v + v^2} - \lambda v}{2v}$ where $u = \sum_{j\neq j^*}d_j$ and $v = \sum_{j\neq j^*}d_j^2$. Therefore for any $\lambda$,
%\begin{equation}
%   |\hat{\alpha}_\lambda \hat{\beta}_{\lambda,j^*} - \hat{\beta}_{OLS,j^*} | \leq \text{max} \Big(\lambda, \frac{\lambda \sqrt{u^2v + v^2} - \lambda v}{2v} \Big) \ . \
%\end{equation} 

%Therefore we have the bound result. For the last piece, observe that $|\hat{\alpha}_\lambda\hat{\beta}_{\lambda, j^*} - \hat{\beta}_{OLS,j*}|$ is equal to:
%\begin{equation}
%        \bigl\lvert (w_1 - 1) \hat{\beta}_{OLS,j^*} + (1 - w_1) s_{j^*} (|\hat{\beta}_{OLS, j^*}|- \lambda)_+ + w_3 s_{j^*} (|\hat{\beta}_{OLS, j^*}| - \lambda)_+ \bigr\rvert \ . \
%\end{equation}
% \begin{align}
%         |\hat{\alpha}_\lambda\hat{\beta}_{\lambda, j^*} - \hat{\beta}_{OLS,j*}| &= \bigl\lvert (w_1 - 1) \hat{\beta}_{OLS,j^*} + (1 - w_1) s_{j^*} (|\hat{\beta}_{OLS, j^*}|- \lambda)_+ \\
%         & \qquad + w_3 s_{j^*} (|\hat{\beta}_{OLS, j^*}| - \lambda)_+ \bigr\rvert \ . \
% \end{align}
%It is simple to show that as $|\hat{\beta}_{OLS, j^*}|$ goes to infinity, $(w_1 - 1) \hat{\beta}_{OLS,j^*}$, $(1 - w_1) s_{j^*} (|\hat{\beta}_{OLS, j^*}| - \lambda)_+$, and $w_2 (|\hat{\beta}_{OLS,j^*}|-\lambda)_+$ all approach 0. Therefore, as $|\hat{\beta}_{OLS, j*}| \rightarrow \infty$, $|\hat{\alpha}_\lambda\hat{\beta}_{j*,\lambda} - \hat{\beta}_{OLS, j*}| \rightarrow 0$.

 
% Note that this bound may be simplified when we apply the Triangle Inequality to the first term in this expression. We find:
% \begin{align}
%   |\hat{\alpha}_\lambda \hat{\beta}_{\lambda,j^*} - \hat{\beta}_{OLS,j^*} | &\leq \frac{\lambda \Big((\sum_{j\neq j^*}d_j)\sqrt{\sum_{j\neq j^*}d_j^2} + \sum_{j\neq j^*}d_j^2 - \sum_{j\neq j^*}d_j^2  \Big)}{2(\sum_{j\neq j^*}d_j^2)}\\
%   &\leq \Big(\frac{\lambda}{2} \Big) \Bigg( \frac{\sum_{j\neq j^*}d_j}{\sqrt{\sum_{j\neq j^*}d_j^2} }\Bigg)
%   %\\
%   %& \leq \frac{\lambda}{2} \left(\frac{k\max(d_j)}{\sqrt{k\max(d_j)^2}} \right)=\frac{\lambda \sqrt{k}}{2}
% \end{align}
% We can see from this bound that as $d_j$ values become large, the bound becomes smaller for a fixed $\lambda$. That is, the larger the signals of our other covariates, the more closely the modified estimates approach the OLS estimates. This bound is especially large when $d_j$ values are close to zero.

% \begin{proof}[Proof of Corollary~\ref{thm:OrthAbsDiffGoesToInf}]
% Observe that $|\hat{\alpha}_\lambda\hat{\beta}_{\lambda, j^*} - \hat{\beta}_{OLS,j*}|$ is equal to:
% \begin{equation}
%         \bigl\lvert (w_1 - 1) \hat{\beta}_{OLS,j^*} + (1 - w_1) s_{j^*} (|\hat{\beta}_{OLS, j^*}|- \lambda)_+ + w_3 s_{j^*} (|\hat{\beta}_{OLS, j^*}| - \lambda)_+ \bigr\rvert \ . \
% \end{equation}
% % \begin{align}
% %         |\hat{\alpha}_\lambda\hat{\beta}_{\lambda, j^*} - \hat{\beta}_{OLS,j*}| &= \bigl\lvert (w_1 - 1) \hat{\beta}_{OLS,j^*} + (1 - w_1) s_{j^*} (|\hat{\beta}_{OLS, j^*}|- \lambda)_+ \\
% %         & \qquad + w_3 s_{j^*} (|\hat{\beta}_{OLS, j^*}| - \lambda)_+ \bigr\rvert \ . \
% % \end{align}
% It is simple to show that as $|\hat{\beta}_{OLS, j^*}|$ goes to infinity, $(w_1 - 1) \hat{\beta}_{OLS,j^*}$, $(1 - w_1) s_{j^*} (|\hat{\beta}_{OLS, j^*}| - \lambda)_+$, and $w_2 (|\hat{\beta}_{OLS,j^*}|-\lambda)_+$ all approach 0. Therefore, as $|\hat{\beta}_{OLS, j*}| \rightarrow \infty$, $|\hat{\alpha}_\lambda\hat{\beta}_{j*,\lambda} - \hat{\beta}_{OLS, j*}| \rightarrow 0$.
% \end{proof}


\begin{proof}[Proof of Theorem~\ref{thm:NonOrthAbsDiff}]
When the sign vector of the true model, $\V{s}$, is known there exists a closed form expression for the non-zero Lasso estimates. Let $\V{s}_1$ be the sign of the non-zero coefficient estimates and $\hat{\boldbeta}_{\lambda,1}$ be the lasso estimates for non-zero coefficients. Then $\hat{\boldbeta}_{\lambda,1} = (\hat{\boldbeta}_{OLS,1} - n\lambda (\V{X}_1^T \V{X}_1)^{-1} \V{s}_1)$ where $\V{X}_1$ is the covariate matrix including all variables $\V{s}_1$ and $\hat{\boldbeta}_{OLS,1} = (\V{X}_1^T\V{X}_1)^{-1}\V{X}_1^T\V{y}$. 
% The following is also known:
% \begin{align}
%     \hat{\alpha}_\lambda \hat{\boldbeta}_{\lambda} &= \Big( \frac{\hat{\boldbeta}_\lambda^T \V{X}_1^T \V{y} }{\hat{\boldbeta}_\lambda^T \V{X}_1^T \V{X}_1 \hat{\boldbeta}_\lambda} \Big) \hat{\boldbeta}_{\lambda}.
% \end{align}
% Now, supposing $\hat{\beta}_{\lambda,j^*} \neq 0$:
% \begin{align}
%   \hat{\V{y}}_\lambda^T \V{y}
%   &= \big( \sum_{i=1}^n x_{ij^*}^2\big)\hat{\beta}_{OLS,j^*}^2 + \big(2\sum_{i=1}^nx_{ij^*}\big(\sum_{j\neq j^*}x_{ij}\hat{\beta}_{OLS,j}\big)\big) - n\lambda s_{j^*} \big)\hat{\beta}_{OLS,j^*}\\ &\hspace{30pt} -n \lambda \sum_{j\neq j^*}|\hat{\beta}_{OLS,j}| + \sum_{i = 1}^n \big(\sum_{j\neq j^*} \hat{\beta}_{OLS,j}x_{ij} \big)^2
% %   \\
%   \end{align}
%   \begin{align}
%   \hat{\V{y}}_\lambda^T \hat{\V{y}}_\lambda &=  \big( \sum_{i=1}^n x_{ij^*}^2\big)\hat{\beta}_{OLS,j^*}^2 + \big(2\sum_{i=1}^nx_{ij^*}\big(\sum_{j\neq j^*}x_{ij}\hat{\beta}_{OLS,j}\big)\big) - 2n\lambda s_{j^*} \big)\hat{\beta}_{OLS,j^*}\\ &\hspace{30pt} -2n \lambda \sum_{j\neq j^*}|\hat{\beta}_{OLS,j}| + \sum_{i = 1}^n \big(\sum_{j\neq j^*} \hat{\beta}_{OLS,j}x_{ij} \big)^2 + n^2\lambda^2 \V{s}_1^T(\V{X}_1^T\V{X}_1)^{-1}\V{s}_1 \ . \
% \end{align} 
%When $x_{ij}$ is the $i$th element of the $j$th column of $\V{X}_1$  
Note that:
\begin{equation}
  \hat{\V{y}}_\lambda^T \V{y} - \hat{\V{y}}_\lambda^T \hat{\V{y}}_\lambda =  n\lambda s_{j^*} \hat{\beta}_{OLS,j^*} + n\lambda \sum_{j\neq j^*}|\hat{\beta}_{OLS,j}| - n^2 \lambda^2 \V{s}^T_1 (\V{X}_1^T \V{X}_1)^{-1} \V{s}_1.
\end{equation}
Hence:
\begin{equation}
    \hat{\alpha}_\lambda \hat{\beta}_{\lambda, j^*} - \hat{\beta}_{OLS, j^*}
    = \frac{(\hat{\V{y}}_\lambda^T \V{y} - \V{y}_\lambda^T \hat{\V{y}}_\lambda)\hat{\beta}_{OLS, j^*} - n\lambda\hat{\V{y}}_\lambda^T \V{y} [(\V{X}_1^T \V{X}_1)^{-1} \V{s}_1]_{j^*}}{\hat{\V{y}}_\lambda^T \hat{\V{y}}_\lambda}\ .\
\end{equation}
Using the expression for $\hat{\V{y}}_\lambda^T \V{y} - \hat{\V{y}}_\lambda^T \hat{\V{y}}_\lambda$ derived above, it can be shown that as $|\hat{\beta}_{OLS,j^*}| \rightarrow \infty$:
% \begin{equation}
%     \hat{\alpha}_\lambda \hat{\beta}_{\lambda, j^*} - \hat{\beta}_{OLS, j^*}
%     \rightarrow  n\lambda \Big( \frac{ s_{j^*}}{\big( \sum_{i=1}^n x_{ij^*}^2\big)} -[(\V{X}_1^T \V{X}_1)^{-1} \V{s}_1]_{j^*}\Big).
% \end{equation}
% If we assume that the columns of $\V{X}$ have been centered and scaled, we can say:
\begin{equation}
  \hat{\alpha}_\lambda \hat{\beta}_{\lambda, j^*} - \hat{\beta}_{OLS, j^*} \rightarrow n\lambda \Big( s_{j^*} -[(\V{X}_1^T \V{X}_1)^{-1}]_{j^*} \V{s}_1\Big) = G \ ,\
\end{equation}
where $[(\V{X}_1^T \V{X}_1)^{-1}]_{j^*}$ denotes the $j^*$-th row of $(\V{X}_1^T \V{X}_1)^{-1}$.
It is simple to show by contradiction that $\lvert G \rvert \leq \lvert \hat{\beta}_{\lambda, j^*} - \hat{\beta}_{OLS, j^*} \rvert .$ \end{proof} %Thus absolute value of the difference $\alpha$-Modified Lasso estimate and the OLS estimate approaches a constant that is always less than the absolute value of the difference between the unmodified Lasso estimate and the OLS estimate as the OLS estimate approaches infinity.




